Numerical methods for computing the discrete and continuous Laplace transforms

We propose a numerical method to spline-interpolate discrete signals and then apply the integral transforms to the corresponding analytical spline functions. This represents a robust and computationally efficient technique for estimating the Laplace transform for noisy data. We revisited a Meijer-G symbolic approach to compute the Laplace transform and alternative approaches to extend canonical observed time-series. A discrete quantization scheme provides the foundation for rapid and reliable estimation of the inverse Laplace transform. We derive theoretic estimates for the inverse Laplace transform of analytic functions and demonstrate empirical results validating the algorithmic performance using observed and simulated data. We also introduce a generalization of the Laplace transform in higher dimensional space-time. We tested the discrete LT algorithm on data sampled from analytic functions with known exact Laplace transforms. The validation of the discrete ILT involves using complex functions with known analytic ILTs.

==> References.tex <==
\section{References}



==> Settings/boldLetters.tex <==
%%!TEX TS-program = pdflatex
%%!TEX encoding = UTF-8 Unicode

% 120 Character width (because 80 just wasn't enough)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 80 --> %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 120 -->

% This file provides bold letters under the \b<letterName> syntax.  If a function is already defined under the same
% name and error will be issued

% Some letters may not render as bold if the fonts don't support it

\NewDocumentCommand{\ba}{}{\mbf{a}}
\NewDocumentCommand{\bb}{}{\mbf{b}}
\NewDocumentCommand{\bc}{}{\mbf{c}}
\NewDocumentCommand{\bd}{}{\mbf{d}}
\NewDocumentCommand{\be}{}{\mbf{e}}
%\NewDocumentCommand{\bf}{}{\mbf{f}}  <--- \bf is already "bold face"
\NewDocumentCommand{\bg}{}{\mbf{g}}
\NewDocumentCommand{\bh}{}{\mbf{h}}
\NewDocumentCommand{\bi}{}{\mbf{i}}
\NewDocumentCommand{\bj}{}{\mbf{j}}
\NewDocumentCommand{\bk}{}{\mbf{k}}
\NewDocumentCommand{\bl}{}{\mbf{l}}
%\NewDocumentCommand{\bm}{}{\mbf{m}}  <--- \bm is already "bold math"
\NewDocumentCommand{\bn}{}{\mbf{n}}
\NewDocumentCommand{\bo}{}{\mbf{o}}
\NewDocumentCommand{\bp}{}{\mbf{p}}
\NewDocumentCommand{\bq}{}{\mbf{q}}
\NewDocumentCommand{\br}{}{\mbf{r}}
\NewDocumentCommand{\bs}{}{\mbf{s}}
\NewDocumentCommand{\bt}{}{\mbf{t}}
\NewDocumentCommand{\bu}{}{\mbf{u}}
\NewDocumentCommand{\bv}{}{\mbf{v}}
\NewDocumentCommand{\bw}{}{\mbf{w}}
\NewDocumentCommand{\bx}{}{\mbf{x}}
\NewDocumentCommand{\by}{}{\mbf{y}}
\NewDocumentCommand{\bz}{}{\mbf{z}}

\NewDocumentCommand{\bA}{}{\mbf{A}}
\NewDocumentCommand{\bB}{}{\mbf{B}}
\NewDocumentCommand{\bC}{}{\mbf{C}}
\NewDocumentCommand{\bD}{}{\mbf{D}}
\NewDocumentCommand{\bE}{}{\mbf{E}}
\NewDocumentCommand{\bF}{}{\mbf{F}}
\NewDocumentCommand{\bG}{}{\mbf{G}}
\NewDocumentCommand{\bH}{}{\mbf{H}}
\NewDocumentCommand{\bI}{}{\mbf{I}}
\NewDocumentCommand{\bJ}{}{\mbf{J}}
\NewDocumentCommand{\bK}{}{\mbf{K}}
\NewDocumentCommand{\bL}{}{\mbf{L}}
\NewDocumentCommand{\bM}{}{\mbf{M}}
\NewDocumentCommand{\bN}{}{\mbf{N}}
\NewDocumentCommand{\bO}{}{\mbf{O}}
\NewDocumentCommand{\bP}{}{\mbf{P}}
\NewDocumentCommand{\bQ}{}{\mbf{Q}}
\NewDocumentCommand{\bR}{}{\mbf{R}}
\NewDocumentCommand{\bS}{}{\mbf{S}}
\NewDocumentCommand{\bT}{}{\mbf{T}}
\NewDocumentCommand{\bU}{}{\mbf{U}}
\NewDocumentCommand{\bV}{}{\mbf{V}}
\NewDocumentCommand{\bW}{}{\mbf{W}}
\NewDocumentCommand{\bX}{}{\mbf{X}}
\NewDocumentCommand{\bY}{}{\mbf{Y}}
\NewDocumentCommand{\bZ}{}{\mbf{Z}}

\NewDocumentCommand{\balpha}{}{\mbf{\alpha}}
\NewDocumentCommand{\bbeta}{}{\mbf{\beta}}
\NewDocumentCommand{\bchi}{}{\mbf{\chi}}
\NewDocumentCommand{\bdelta}{}{\mbf{\delta}}
\NewDocumentCommand{\bepsilon}{}{\mbf{\epsilon}}
%\NewDocumentCommand{\beta}{}{\mbf{\eta}}		<--- \beta is already a symbol
\NewDocumentCommand{\bgamma}{}{\mbf{\gamma}}
\NewDocumentCommand{\biota}{}{\mbf{\iota}}
\NewDocumentCommand{\bkappa}{}{\mbf{\kappa}}
\NewDocumentCommand{\blambda}{}{\mbf{\lambda}}
\NewDocumentCommand{\bmu}{}{\mbf{\mu}}
\NewDocumentCommand{\bnu}{}{\mbf{\nu}}
\NewDocumentCommand{\bomega}{}{\mbf{\omega}}
\NewDocumentCommand{\bphi}{}{\mbf{\phi}}
\NewDocumentCommand{\bpi}{}{\mbf{\pi}}
\NewDocumentCommand{\bpsi}{}{\mbf{\psi}}
\NewDocumentCommand{\brho}{}{\mbf{\rho}}
\NewDocumentCommand{\bsigma}{}{\mbf{\sigma}}
\NewDocumentCommand{\btau}{}{\mbf{\tau}}
\NewDocumentCommand{\btheta}{}{\mbf{\theta}}
\NewDocumentCommand{\bupsilon}{}{\mbf{\upsilon}}
\NewDocumentCommand{\bvarepsilon}{}{\mbf{\varepsilon}}
\NewDocumentCommand{\bvarpi}{}{\mbf{\varpi}}
\NewDocumentCommand{\bvarphi}{}{\mbf{\varphi}}
\NewDocumentCommand{\bvarrho}{}{\mbf{\varrho}}
\NewDocumentCommand{\bvarsigma}{}{\mbf{\varsigma}}
\NewDocumentCommand{\bvartheta}{}{\mbf{\vartheta}}
\NewDocumentCommand{\bxi}{}{\mbf{\xi}}
\NewDocumentCommand{\bzeta}{}{\mbf{\zeta}}

\NewDocumentCommand{\bDelta}{}{\mbf{\Delta}}
\NewDocumentCommand{\bGamma}{}{\mbf{\Gamma}}
\NewDocumentCommand{\bLambda}{}{\mbf{\Lambda}}
\NewDocumentCommand{\bOmega}{}{\mbf{\Omega}}
\NewDocumentCommand{\bPhi}{}{\mbf{\Phi}}
\NewDocumentCommand{\bPi}{}{\mbf{\Pi}}
\NewDocumentCommand{\bPsi}{}{\mbf{\Psi}}
\NewDocumentCommand{\bSigma}{}{\mbf{\Sigma}}
\NewDocumentCommand{\bTheta}{}{\mbf{\Theta}}
\NewDocumentCommand{\bUpsilon}{}{\mbf{\Upsilon}}
\NewDocumentCommand{\bXi}{}{\mbf{\Xi}}



==> Settings/commonDefinitions.tex <==
%! program = pdflatex

% This file contains definitions commonly used in my memos.

% Bold
\newcommand{\mbf}[1]{\ensuremath{\bm{#1}}}

% Abs
\newcommand{\abs}[1]{\ensuremath{\left| #1 \right|}}

% Norm
\newcommand{\norm}[1]{\ensuremath{\left\| #1 \right\|}}

% Span
%\newcommand{\span}[1]{\mathrm{span}\of{#1}}

% Kron
\newcommand{\kron}{\ensuremath{\otimes}}

% Del
\newcommand{\del}{\ensuremath{\ \nabla}}

% MATLAB
\newcommand{\MATLAB}{\ensuremath{\textrm{MATLAB}^\circledR}}



% Col (vec)
\NewDocumentCommand\col{g}{%
  \IfNoValueTF{#1}{\ensuremath{\mathrm{vec}}}{\ensuremath{\mathrm{vec}}\of{#1}}%
}

% "Of" operator 
\NewDocumentCommand\of{og}{%
  \IfNoValueTF{#1}%
    { \IfNoValueTF{#2}{}{\!\({#2}\)} }%
    { \IfNoValueTF{#2}{\!\[{#1}\]}{\!\{{#2}\}} }%
}

% differential
%\DeclareMathOperator{\Diff}{\raisebox{-.09em}{\ipaclap{D}{\raisebox{.204em}{\textpalhook}\kern.45em}}\!}
\DeclareMathOperator{\Diff}{\ipaclap{D}{\raisebox{.204em}{\textpalhook}\kern.44em}\kern-.1em}
\NewDocumentCommand\diff{g}{%
  \IfNoValueTF{#1}
  {\text{\texthtd}}
  {\text{\texthtd}\of{#1}}%
}

% Natural log
\RenewDocumentCommand\ln{g}{%
  \IfNoValueTF{#1}{\mathrm{ln\ }}{\mathrm{ln}\of{#1}}%
}

% Real and imaginary parts as operators
\NewDocumentCommand\Real{og}{%
  \IfNoValueTF{#1}%
    { \IfNoValueTF{#2}{\mathcal{R}\!\!\mathpzc{e}}{\mathcal{R}\!\!\mathpzc{e}\!\{{#2}\}} }%
    { \IfNoValueTF{#2}{\mathcal{R}\!\!\mathpzc{e}\!\[{#1}\]}{\mathcal{R}\!\!\mathpzc{e}\!\({#2}\)} }%
}
\NewDocumentCommand\Imag{og}{%
  \IfNoValueTF{#1}%
    { \IfNoValueTF{#2}{\mathcal{I}\!\!\mathpzc{m}}{\mathcal{I}\!\!\mathpzc{m}\!\{{#2}\}} }%
    { \IfNoValueTF{#2}{\mathcal{I}\!\!\mathpzc{m}\!\[{#1}\]}{\mathcal{I}\!\!\mathpzc{m}\!\({#2}\)} }%
}

% Trigometric Functions
\RenewDocumentCommand\cos{g}{%
  \IfNoValueTF{#1}{\mathrm{cos}}{\mathrm{cos}\of{#1}}%
}
\RenewDocumentCommand\sin{g}{%
  \IfNoValueTF{#1}{\mathrm{sin}}{\mathrm{sin}\of{#1}}%
}
\RenewDocumentCommand\tan{g}{%
  \IfNoValueTF{#1}{\mathrm{tan}}{\mathrm{tan}\of{#1}}%
}
\RenewDocumentCommand\arccos{g}{%
  \IfNoValueTF{#1}{\mathrm{arccos}}{\mathrm{arccos}\of{#1}}%
}
\RenewDocumentCommand\arcsin{g}{%
  \IfNoValueTF{#1}{\mathrm{arcsin}}{\mathrm{arcsin}\of{#1}}%
}
\RenewDocumentCommand\arctan{g}{%
  \IfNoValueTF{#1}{\mathrm{arctan}}{\mathrm{arctan}\of{#1}}%
}
\RenewDocumentCommand\cot{g}{%
  \IfNoValueTF{#1}{\mathrm{cot}}{\mathrm{cot}\of{#1}}%
}

% Floor and Ceil
\newcommand{\floor}[1]{\ensuremath{\left\lfloor #1 \right\rfloor}}
\newcommand{\ceil}[1]{\ensuremath{\left\lceil #1 \right\rceil}}

% s.t. (such that)
\newcommand{\st}[1][14pt]{\text{\ \hspace{#1} s.t. \hspace{#1}}}

% tr
\NewDocumentCommand\tr{g}{%
  \IfNoValueTF{#1}{\mathrm{tr}}{\mathrm{tr}\of{#1}}%
}

% sgn
\newcommand{\sgn}[1]{\mathrm{sgn}\of{#1}}

% diag
\NewDocumentCommand\diag{og}{%
  \IfNoValueTF{#1}%
    { \IfNoValueTF{#2}{\ensuremath{\mathrm{diag}}}{\ensuremath{\mathrm{diag}\of{#2}}} }%
    { \IfNoValueTF{#2}{\ensuremath{\mathrm{diag}\of[#1]}}{\ensuremath{\mathrm{diag}\of[]{#2}}} }%
}

% exp
\RenewDocumentCommand\exp{g}{%
  \IfNoValueTF{#1}{\ensuremath{\mathrm{exp}}}{\ensuremath{\mathrm{exp}}\of{#1}}%
}

% ierf
\DeclareMathOperator{\ierf}{ierf}

% shah
\DeclareMathOperator{\shah}{\uparrow\joinrel\uparrow\joinrel\uparrow}

% derivative ... i.e. \deriv{f}{x}  or \deriv[2]{f}{x,y}
\newcommand{\deriv}[3][{{}\mspace{-2mu}}]{\ensuremath{\frac{\partial^#1#2}{\foreach{\partial}{}{#3}}}}

% Probability and remap the paragraph marker to \Par
\newcommand{\p}[2][]{\ensuremath{p_{#1}\left( #2 \right)}}
\let\Par\P
\renewcommand{\P}[2][]{\ensuremath{P_{#1}\left( #2 \right)}}

% Operator {2}_{1}[{3}]
\newcommand{\Operator}[3][]{\ensuremath{{\mathrm{#2}}_{#1}\!\left[ #3 \right]}}

% Expectation
\newcommand{\E}[2][]{\Operator[#1]{E}{#2}}

% Variance
\newcommand{\Var}[2][]{\Operator[#1]{Var}{#2}}

% Correlation
\newcommand{\R}[2][]{\Operator[#1]{R}{#2}}

% Covariance
%\newcommand{\C}[2][]{\Operator[#1]{Cov}{#2}}
\NewDocumentCommand\C{g}{%
  \IfNoValueTF{#1}{\mathrm{Cov}}{\mathrm{Cov}\of{#1}}%
}
% Bias
\newcommand{\bias}[2][]{\Operator[#1]{bias}{#2}}

% MSE
\newcommand{\MSE}[2][]{\Operator[#1]{MSE}{#2}}

% Kullback-Leibler
\newcommand{\K}[2][]{\Operator[#1]{K}{#2}}

% Entropy and cross-entropy
%\newcommand{\H}[2][]{\Operator[#1]{K}{#2}}

% Inner product
\newcommand{\inner}[2]{\left \langle {#1} \ , \ {#2} \right \rangle}

% rank
\newcommand{\rank}[1]{\text{rank}\of{#1}}

% Parentheses and brackets
% Use \math or $ to enable a math environment
\renewcommand{\(}{\ensuremath{\left(}}
\renewcommand{\)}{\ensuremath{\right)}}
\renewcommand{\[}{\ensuremath{\left[}}
\renewcommand{\]}{\ensuremath{\right]}}
\newcommand{\<}{\ensuremath{\left<}}
\renewcommand{\>}{\ensuremath{\right>}}
\let\oldBracketLeft\{
\let\oldBracketRight\}
\renewcommand{\{}{\ensuremath{\left\oldBracketLeft}}
\renewcommand{\}}{\ensuremath{\right\oldBracketRight}}

% max and min functions
%\RenewDocumentCommand\max{g}{%
%  \IfNoValueTF{#1}{\mathrm{max\ }}{\mathrm{max}\of{#1}}%
%}
%\RenewDocumentCommand\min{g}{%
%  \IfNoValueTF{#1}{\mathrm{min\ }}{\mathrm{min}\of{#1}}%
%}

% Argmax, Argmin, minmax, maxmin,...
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\minmax}{min\,max}
\DeclareMathOperator*{\maxmin}{max\,min}
\DeclareMathOperator*{\argsup}{arg\,sup}
\DeclareMathOperator*{\esssup}{ess\,sup}

% Greater than less than (better way to do this???)
\DeclareMathOperator*{\gtlt}{\ensuremath{\begin{array}{c} > \vspace{-6pt} \\ < \end{array}}}

% Fourier Transform Operator
\NewDocumentCommand\F{og}{%
  \IfNoValueTF{#1}%
    { \IfNoValueTF{#2}{\mathcal{F}}{\mathcal{F}\!\{{#2}\}} }%
    { \IfNoValueTF{#2}{\mathcal{F}\!\[{#1}\]}{\mathcal{F}\!\({#2}\)} }%
}
\NewDocumentCommand\FInv{og}{%
  \IfNoValueTF{#1}%
    { \IfNoValueTF{#2}{\mathcal{F}^{-1}}{\mathcal{F}^{-1}\!\{{#2}\}} }%
    { \IfNoValueTF{#2}{\mathcal{F}^{-1}\!\[{#1}\]}{\mathcal{F}^{-1}\!\({#2}\)} }%
}


% erf
\DeclareMathOperator{\erf}{erf}

% rect
\NewDocumentCommand\rect{g}{%
  \IfNoValueTF{#1}
  {\ensuremath{\mathrm{rect}}}
  {\ensuremath{\mathrm{rect}\of{#1}}}%
}

% sinc
\NewDocumentCommand\sinc{g}{%
  \IfNoValueTF{#1}
  {\ensuremath{\mathrm{sinc}}}
  {\ensuremath{\mathrm{sinc}\of{#1}}}%
}

% sin, cos, tan, cot, arcsin


% circ
\DeclareMathOperator{\Circ}{Circ}

% supp
\NewDocumentCommand\supp{g}{%
  \IfNoValueTF{#1}
  {\ensuremath{\mathrm{supp}}}
  {\ensuremath{\mathrm{supp}\of{#1}}}%
}


% defeq
\DeclareMathOperator*{\defeq}{\stackrel{\mathrm{def}}{=}}

% Calligraphy
\let\oldMathcal\mathcal
\renewcommand{\mathcal}[1]{\ensuremath{\oldMathcal{#1}}}

% Insert Blank Page  (need help here)
%\makeatletter \ifodd\c@page \pagebreak \else \newpage \text{\thispagestyle{empty}} \newpage \fi \makeatother

\makeatletter
% Functional foreach construct 
% #1 - Function to call on each comma-separated item in #3
% #2 - Parameter to pass to function in #1 as first parameter (constant)
% #3 - Comma-separated list of items to pass as second parameter to function #1
\def\foreach#1#2#3{%
  \@test@foreach{#1}{#2}#3,\@end@token
}

% Internal helper function - Eats one input
\def\@swallow#1{}

% Internal helper function - Checks the next character after #1 and #2 and 
% continues loop iteration if \@end@token is not found 
\def\@test@foreach#1#2{%
  \@ifnextchar\@end@token%
    {\@swallow}%
    {\@foreach{#1}{#2}}%
}

% Internal helper function - Calls #1{#2}{#3} and recurses
% The magic of splitting the third parameter occurs in the pattern matching of the \def
\def\@foreach#1#2#3,#4\@end@token{%
  #1{#2}{#3}%
  \@test@foreach{#1}{#2}#4\@end@token%
}
\makeatother


